Geometry, Computation, and Optimality in Stochastic Optimization

We study computational and statistical consequences of problem geometry in stochastic and online optimization. By focusing on constraint set and gradient geometry, we characterize the problem families for which stochastic- and adaptive-gradient methods are (minimax) optimal and, conversely, when nonlinear updates -- such as those mirror descent employs -- are necessary for optimal convergence. When the constraint set is quadratically convex, diagonally pre-conditioned stochastic gradient methods are minimax optimal. We provide quantitative converses showing that the ``distance'' of the underlying constraints from quadratic convexity determines the sub-optimality of subgradient methods. These results apply, for example, to any $\ell_p$-ball for $p < 2$, and the computation/accuracy tradeoffs they demonstrate exhibit a striking analogy to those in Gaussian sequence models.

==> informs-proof-macro.tex <==
% -*- mode: latex -*- %

% This fixes it so \begin{proof} and \end{proof} work with Informs style.

\makeatletter  % Make example environment indented as a list, about 1em
\renewenvironment{proof}{%
  \list{}{%
    \itemindent\parindent
    \leftmargin0em  % Amount to indent whole example
    \rightmargin\leftmargin  % Set right margin same as left
    \parsep\z@\@plus\p@  % Separate paragraphs
    \listparindent\parindent % Indent new paragraphs
  }%
\item\relax % No number on the item
  \noindent \hspace*{1em}\textit{Proof.}\hspace*{.05em}
  % There is no text to display in the example
}{%
  $\Halmos$ \endlist
}
\makeatother

\usepackage{xifthen}

\makeatletter  % Make example environment indented as a list, about 1em
\renewenvironment{example}[1][]{%
  \refstepcounter{example}
  \list{}{%
    \itemindent\parindent
    \leftmargin0em  % Amount to indent whole example
    \rightmargin\leftmargin  % Set right margin same as left
    \parsep\z@\@plus\p@  % Separate paragraphs
    \listparindent\parindent % Indent new paragraphs
  }%
\item\relax % No number on the item
  \ifthenelse{\isempty{#1}}{%
    % There is no text to display in the example
    {\sffamily\mdseries\scshape Example \theexample.}\hspace*{.05em}
  }{%
    % There is text
    {\sffamily\mdseries\scshape Example \theexample ({#1}).}\hspace*{.05em}
  }
}{%
  $\Diamond$ \endlist
}
\makeatother


==> moor-prelims.tex <==
% -*- mode: latex -*- %

% Document preliminaries for the Math of OR submission

\usepackage{eqndefns-left} % For checking the display equation width and
                           % equation environment definitions %
\RequirePackage{tgtermes}
\RequirePackage{newtxtext}
\RequirePackage{newtxmath}
% \RequirePackage{bm}
\RequirePackage{endnotes}

%\OneAndAHalfSpacedXI
\OneAndAHalfSpacedXII % Current default line spacing
%%\DoubleSpacedXI
%%\DoubleSpacedXII

% Natbib setup for author-number style
\usepackage[sort&compress]{natbib}
\bibpunct[, ]{[}{]}{,}{n}{}{,}%
\def\bibfont{\small}%
\def\bibsep{\smallskipamount}%
\def\bibhang{24pt}%
\def\newblock{\ }%
\def\BIBand{and}%

%% Setup of the equation numbering system. Outcomment only one.
%% Preferred default is the first option.
\EquationsNumberedThrough    % Default: (1), (2), ...
%\EquationsNumberedBySection % (1.1), (1.2), ...

%% Setup of theorem styles. Outcomment only one.
%% Preferred default is the first option.
\TheoremsNumberedThrough     % Preferred (Theorem 1, Lemma 1, Theorem 2)
%\TheoremsNumberedByChapter  % (Theorem 1.1, Lema 1.1, Theorem 1.2)
\ECRepeatTheorems  %  

% For new submissions, leave this number blank.
% For revisions, input the manuscript number assigned by the on-line
% system along with a suffix ".Rx" where x is the revision number.
\MANUSCRIPTNO{}

\input{informs-proof-macro}

% Author's names for the running heads
% Sample depending on the number of authors;
% \RUNAUTHOR{Jones}
% \RUNAUTHOR{Jones and Wilson}
% \RUNAUTHOR{Jones, Miller, and Wilson}
% \RUNAUTHOR{Jones et al.} % for four or more authors
% Enter authors following the given pattern:
%\RUNAUTHOR{}
\RUNAUTHOR{Cheng, Duchi and Levy}

% Title or shortened title suitable for running heads. Sample:
% \RUNTITLE{Predictive Maintenance in Manufacturing}
% Enter the (shortened) title:
\RUNTITLE{Geometry, Computation, and Optimality in Stochastic Optimization}

% Full title. Sample:
% \TITLE{Optimal Resource Allocation in Humanitarian Logistics: A Stochastic Programming Approach}
% Enter the full title:
\TITLE{Geometry, Computation, and Optimality in Stochastic Optimization}

% Block of authors and their affiliations starts here:
% NOTE: Authors with same affiliation, if the order of authors allows,
%   should be entered in ONE field, separated by a comma.
%   \EMAIL field can be repeated if more than one author
\ARTICLEAUTHORS{%
  \AUTHOR{Chen Cheng}
  \AFF{Department of Statistics,
    Stanford University, \EMAIL{chencheng@stanford.edu}}
  
  \AUTHOR{John C.\ Duchi}
  \AFF{Departments of Statistics and Electrical Engineering,
    Stanford University, \EMAIL{jduchi@stanford.edu}}
  
  \AUTHOR{Daniel Levy}
  \AFF{Department of Computer Science,
    Stanford University, \EMAIL{danilevy@stanford.edu}}
  % Enter all authors
} % end of the block

\ABSTRACT{%
  \input{abstract}
}%

\FUNDING{JCD, CC, and DL partially supported
  by NSF-CAREER Award 1553086, ONR-YIP N00014-19-1-2288,
  and the Stanford DAWN Project. JCD and CC additionally
  supported by NSF Award IIS-2006777 and
  ONR Award N00014-22-1-2669.}

%Supplemental Material:
%Data Ethics & Reproducibility Note:

% Sample
%\KEYWORDS{Stochastic programming, Decision support,Uncertainty, Disaster response, Optimization}

% Fill in data. If unknown, outcomment the field
\KEYWORDS{Geometry, Computational Optimality, Stochastic Optimization, Gaussian Sequence Models} 

